Stabilization and Optimal Control of an Interconnected $n + m$ Hetero-directional Hyperbolic PDE-SDE System

In this paper, we design a controller for an interconnected system composed of a linear Stochastic Differential Equation (SDE) controlled through a linear hetero-directional hyperbolic Partial Differential Equation (PDE). Our objective is to steer the coupled system to a desired final state on average, while keeping the variance-in-time as small as possible, improving robustness to disturbances. By employing backstepping techniques, we decouple the original PDE, reformulating the system as an input delayed SDE with a stochastic drift. We first establish a controllability result, shading light on lower bounds for the variance. This shows that the system can never improve variance below strict structural limits. Under standard controllability conditions, we then design a controller that drives the mean of the states while keeping the variance bounded. Finally, we analyze the optimal control problem of variance minimization along the entire trajectory. Under additional controllability assumptions, we prove that the optimal control can achieve any variance level above the fundamental structural limit.

==> 03_Tracking_Problem.tex <==


%In system \eqref{eq:coupled_PDE_SDE}, the in-domain coupling terms $\Sigma^{\cdot\cdot}$ in the PDE can cause instabilities and disrupt the control of the SDE \cite{auriol_delay-robust_2018}. %\modifJA{Mettre une citation?}. 
%Therefore, we will first apply a backstepping transformation to move these coupling terms to the boundary at $x=1$, where the control input is applied. Then, we will design the input $V(t)$ as a sum of two control components: $V(t)=\VPDE(t)+\Veff(t)$. The term $\VPDE(t)$ will correspond to a classical backstepping control input,  used to cancel the (potentially) unstable coupling terms appearing at the controlled boundary. It would stabilize the PDE in the absence of the SDE. On the other hand, $\Veff(t)$ is the effective control that propagates through the PDE, allowing us to track a desired signal entering the SDE.


In system \eqref{eq:coupled_PDE_SDE}, the in-domain coupling terms $\Sigma^{\cdot\cdot}$ in the PDE may cause instabilities and disrupt the control of the SDE \cite{auriol_delay-robust_2018}. %\modifJA{Mettre une citation?}. 
Our idea to cope with this challenge is to apply backstepping in the first place to move these coupling terms to the boundary at $x=1$, where the control input is applied. Then, we will design the input $V(t)$ as a sum of two control components: $V(t)=\VPDE(t)+\Veff(t)$. The term $\VPDE(t)$ will correspond to a classical backstepping control input,  used to cancel the (potentially) unstable coupling terms appearing at the controlled boundary. It would stabilize the PDE in the absence of the SDE. On the other hand, $\Veff(t)$ is the effective control that propagates through the PDE, allowing us to track a desired signal entering the SDE. %This allows us to use stochastic control tools to handle the equivalent input delayed SDE.


%\modifJA{J'ai bougé la fin ailleurs car ça faisait trop de choses à assimiler.}



%\subsection{Transformation into a Target System}
%\subsubsection{The Backstepping Transformation}
%\subsubsection{Existence of a Solution of the Kernel Equations}

\subsection{The Backstepping Transformation}

Taking inspiration from \cite{auriol_delay-robust_2018}, we consider the following backstepping change of variables:

\begin{equation}\label{eq:backstepping_transform_alpha_beta_definition}
 \begin{split}
 \alpha(t,x) \triangleq u(t,x) & + \int_0^x K_{uu}(x,y) u(t,y) dy \\ 
 & + \int_0^x K_{uv}(x,y) v(t,y) dy + \gamma_\alpha(x) X(t) \\
 \beta(t,x) \triangleq v(t,x) & + \int_0^x K_{vu}(x,y) u(t,y) dy \\ 
 & + \int_0^x K_{vv}(x,y) v(t,y) dy + \gamma_\beta(x) X(t).
 \end{split}
\end{equation}
The kernels  $K_{uu}, K_{uv}, K_{vu}$, and $K_{vv}$ are piecewise continuous functions defined on the triangular domain $\mathcal{T} \triangleq \left\{ (x,y), x \in [0,1], y \in [0,x]  \right\}$, whereas $\gamma_\alpha, \gamma_\beta$ are in $C^1([0,1] ; \mathbb{R}^{n \times N}) \times C^1([0,1] ; \mathbb{R}^{m \times N})$. On their respective domains of definition, $K$ and $\gamma$ verify the following set of \textit{kernel equations}: 

%\commentGV{Changement d'ordre par rapport à CDC, on introduit d'abord le target système pour introduire les fonctions $\Psi$ et $\Omega$.}





 \begin{equation}\label{eq:kernel_equations_alpha}
 \left\{
 \begin{array}{l}
      \Lambda^+ (K_{uu})_x(x,y) + (K_{uu})_y(x,y) \Lambda^+ \\ 
      \quad + K_{uu}(x,y) \Sigma^{++}(y) + K_{uv}(x,y) \Sigma^{-+}(y) = \Psi(x) K_{uu}(x,y) \\
      \Lambda^+ (K_{uv})_x(x,y) - (K_{uv})_y(x,y) \Lambda^- \\
      \quad + K_{uu}(x,y) \Sigma^{+-}(y) + K_{uv}(x,y) \Sigma^{--}(y) =  \Psi(x) K_{uv}(x,y) \\
      \Lambda^+  K_{uu}(x,x) - K_{uu}(x,x) \Lambda^+ + \Sigma^{++}(x) = 0 \\
      \Lambda^+  K_{uv}(x,x) + K_{uv}(x,x) \Lambda^- + \Sigma^{+-}(x) = 0 \\
      K_{uu}(x,0) \Lambda^+ Q - K_{uv}(x,0) \Lambda^- + \gamma_\alpha(x) B = \Psi(x)  \\
      \Lambda^+ \gamma_\alpha'(x) + \gamma_\alpha(x) A + K_{uu}(x,0) \Lambda^+ M  = 0 \\
      \gamma_\alpha(0) = -M,
 \end{array} 
 \right.
 \end{equation}
 as well as
\modifJA{S'il faut gagner de la place, on pourra utiliser la forme condensée proposée dans LCSS ou mon papier Automatica de 2023 (robustification of ...)} \begin{equation}\label{eq:kernel_equations_beta}
 \left\{
 \begin{array}{l}
      - \Lambda^- (K_{vu})_x(x,y) + (K_{vu})_y(x,y) \Lambda^+ \\
      \quad + K_{vu}(x,y) \Sigma^{++}(y) + K_{vv}(x,y) \Sigma^{-+}(y) = \Omega(x) K_{vu}(x,y) \\
      - \Lambda^- (K_{vv})_x(x,y) - (K_{vv})_y(x,y) \Lambda^- \\
      \quad + K_{vu}(x,y) \Sigma^{+-}(y) + K_{vv}(x,y) \Sigma^{++}(y) = \Omega(x) K_{vv}(x,y) \\
      - \Lambda^-  K_{vu}(x,x) - K_{vu}(x,x) \Lambda^+ + \Sigma^{-+}(x) = 0 \\
      - \Lambda^-  K_{vv}(x,x) + K_{vv}(x,x) \Lambda^- + \Sigma^{--}(x) = \Omega(x) \\
      K_{vu}(x,0) \Lambda^+ Q - K_{vv}(x,0) \Lambda^- + \gamma_\beta(x) B = 0 \\
      - \Lambda^- \gamma_\beta'(x) + \gamma_\beta(x) A  + K_{vu}(x,0) \Lambda^+ M = 0 \\
      \gamma_\beta(0) = 0.
 \end{array} 
 \right.
 \end{equation}
%\commentGV{retrouver ou interviennent $\Psi$ et $\Omega$, les équations ne sont pas bien posées telles qu'elles sont.}
where $\Psi$ and $\Omega$ are two strict upper triangular matrices. %of the form \modifJA{Pas nécessaire de metttre explicitement les matrices. Tu dis déjà qu'elles sont trig. sup.}
% \small
% $$
% \Psi(x) = \left( \begin{array}{ccc} 0 & & (\psi(x))_{i,j} \\ & \ddots &  \\ (0) & & 0 \end{array} \right),  \Omega(x) = \left( \begin{array}{ccc} 0 & & (\omega(x)))_{i,j} \\ & \ddots &  \\ (0) & & 0 \end{array} \right).
% $$
% \normalsize
Their coefficients verify
\begin{align*}
\psi_{i,j}(x) & =  ( \lambda_i - \lambda_j) K_{uu}(x,x)_{i,j} + \Sigma^{++}_{i,j} \\
\omega_{i,j}(x) & = ( \mu_j - \mu_i) K_{vv}(x,x)_{i,j} + \Sigma^{--}_{i,j}.
\end{align*}
The set of equations \eqref{eq:kernel_equations_alpha}-\eqref{eq:kernel_equations_beta}is well posed and admits a unique solution \cite{auriol_minimum_2016, di_meglio_stabilization_2018}. % \modifJA{Il faudrait faire référence au numéro d'équations. Par ailleurs in me semble qu'il y a un problème de conditions de bords pour $K_{uu}(x,0)$. Ca pourrait avoir des conséquence importantes sur le système cible (mais mineures sur le reste du papier). Il faudrait je pense remplacer $\Psi(x)\alpha(t,x)$ par $\Psi(x)\beta(t,0)$ En ref, il faut aussi citer le papier de Di Meglio/Hu/Bribiesca-Argomedo/Krstic (gestion du term ODE).}
By setting our stabilizing backstepping controller as 
\begin{equation}\label{eq:definition_expression_backstep_controller}
\begin{split}
& \VPDE(t) = - R u(t,1) - \gamma_\beta(1) X(t) \\
    & \ - \int_0^1 K_{vu}(1,y) u(t,y) dy - \int_0^1 K_{vv}(1,y) v(t,y) dy.
\end{split}
\end{equation}
and by differentiating with respect to time and space (in the sense of distributions), and integrating by parts, we can show that the states $(\alpha,\beta,X)$ are solutions to the following \textit{target system}:
\begin{equation}\label{eq:first_target_system_SPDE}
\left\{
\begin{array}{l}
     dX(t) = ( A X(t) + B \beta(t,0) ) dt + \sigma(t) dW_t \\
     d \alpha(t,x) + \Lambda^+ \alpha_x(t,x) = \Psi(x)\beta(t,0) + \gamma_\alpha(x) \sigma(t) dW_t \\
     d \beta(t,x) - \Lambda^- \beta_x(t,x) = \Omega(x) \beta(t,x) + \gamma_\beta(x) \sigma(t) dW_t \\
     \alpha(t,0) = Q \beta(t,0), \ \beta(t,1) = \Veff(t) 
\end{array} 
\right.
\end{equation}

%\modifJA{Mettre ce qui suit en remarque:
In the absence of the SDE, this target system would be exponentially stable. However, due to the cancellation of the term $Ru(t,1)$, the feedback operator induced by $\VPDE$ is not strictly proper. This could lead to (delay)-robustness issues, as highlighted in~\cite{auriol_delay-robust_2018}. To address these concerns, different approaches have been proposed as partial cancellation of the reflection~\cite{auriol_delay-robust_2018} or filtering methods~\cite{auriol_robustification_2023}. However, these methods do not directly adapt to the current stochastic configuration. Specifically, we should be able to show robust mean square stability, but quantifying the impact of these techniques on variance proves to be challenging. As our analysis is essentially theoretical, this robustness analysis for a practical implementation is beyond the scope of this paper and is left for future research.
%}

%\revAns{Attention à introduire Vin, Veff et VBS comme dans CDC dans le problem formulation.}

%\subsection{Signal Tracking}

%Although the coupling between $u$ and $v$ is handled, there remain cascading interactions between the states $v^{(i)}(t,x)$ and $v^{(j)}(t,x)$ for $i>j$. 
%Additionally, we need to account for the interaction from the SDE back into the PDE. 
While system \eqref{eq:first_target_system_SPDE} is simpler to handle, expressing $\beta(t,0)$ in terms of $\Veff$ remains complex, hindering the task of tracking a desired control through the PDE into the SDE. In what follows, we show how we can further simplify system   \eqref{eq:first_target_system_SPDE} into an input-delayed SDE, with an arbitrary input $\VSDE \in L^2_\mathcal{F}([0,T] ; \mathbb{R}^m)$ by choosing an appropriate controller $\Veff$.
%We therefore show that, for any desired signal $V_{SDE}(t)$ in $L^2_\mathcal{F}([0,T] ; \mathbb{R}^m)$ that we want to track into the SDE,  $\Veff(t)$ can be chosen to ensure the boundary condition $v^{(i)}(t,0) = V_{SDE}^{(i)}(t-\frac{1}{\mu_i}) + \int_{t - \frac{1}{\mu_i}}^t G_i(t-s ) \sigma(s) dW_s $ is met. The delay reflects the finite control velocity, and the stochastic integral arises from the noise that cannot be canceled.
%\modifJA{$\VSDE$ n'est pas proprement défini. On ne comprend pas à quoi ça correspond.}


\subsection{Solving the SPDE Through the Characteristic Method}
%\modifJA{Balise à garder pour me rappeler de relire cette section une fois modifiée.}


To achieve our desired control behavior at the boundary of the SDE, we start by considering an input $\Veff$ applied to the PDE. Due to the coupling terms within the PDE in system \eqref{eq:first_target_system_SPDE}, this input does not directly translate into a simple expression for $\beta(t,0)$. However, we find that by choosing $\Veff$ of a specific form relative to an arbitrary process $S(t) \in L^2_\mathcal{F}([0,T] ; \mathbb{R}^m)$, we obtain a clean boundary condition at the other end of the PDE $\beta^{(i)}(t,0) = S^{(i)}(t-\frac{1}{\mu_i}) + \int_{t - \frac{1}{\mu_i}}^t G_i(t-s ) \sigma(s) dW_s $.
We will show that this result implies that any desired control $\VSDE$ can be approximately tracked at $\beta(t,0)$ when choosing $S(t) = \VSDE(t)$. 
%We cannot track the process any better, as the delay reflects the finite control velocity, and the stochastic integral arises from the noise that cannot be canceled.
%We can now solve through the characteristic method and the Ito formula the SPDE \eqref{eq:first_target_system_SPDE}. As mentioned previously, this allows us to compute an effective control $\Veff$ that tracks a desired control $\VSDE$ into the SDE.
%For clarity and conciseness, we only do this for $\beta$. %, although a very similar formula can be obtained for $\alpha$.
%\modifJA{Paragraphe peu clair. A reformuler. Pourquoi on a besoin de celle de $\alpha$?}
%\commentGV{A REVOIR: l'expression du contrôle $\Veff$ ne peut pas dépendre de $x$! Il faut en fait prendre l'expression en $x=0$. Le problème c'est que l'expression de $\beta(t,x)$ va changer sur le reste du domaine et on aura une induction qui sera plus complexe que ça. La méthode reste correcte, mais l'expression de $\Veff$ est beaucoup plus compliqué.}
%\commentGV{A REVOIR: Le contrôleur proposé n'est pas causal, il faut revoir la preuve et affiner l'expression de $\beta$.      }
\begin{lemma}\label{lem:track_VSDE_with_Veff_and_formula_beta}
    Let $\VSDE$ be a $ L^2_\mathcal{F}([0,T] ; \mathbb{R}^m)$ controller we want to track into the SDE. %\modifJA{Qu'est-ce que ça veut dire ? Il faut introduire $\VSDE$ plus clairement et proprement.} 
    The input $\Veff \in  L^2_\mathcal{F}([0,T] ; \mathbb{R}^m)$ recursively defined as 
    %such that \modifJA{Domaine de $t$ et $x$?}
    \small
\begin{equation}\label{eq:def_of_Veff_in_terms_of_VSDE}
\begin{split}
% &  \Veff^{(m)}(t)  = \VSDE^{(m)}(t)   \\
% & \Veff^{(i)}(t)  = \VSDE^{(i)} \left(t \right) \\
% & - \sum_{j=i+1}^m  \int_{0}^{\frac{1-x}{\mu_i}} \omega_{i,j}(x + \mu_i s ) \times \\
% & \hspace{6em} \VSDE^{(j)} \left(t + \frac{1-x}{\mu_i} + s - \frac{1 - x - \mu_i s}{\mu_j} \right)  ds 
\Veff^{(i)}(t- \frac{1}{\mu_i} ) & = \VSDE^{(i)}(t- \frac{1}{\mu_i} ) \\
& -  \sum_{j=i+1}^m \int_0^{\frac{1}{\mu_i}} F_{ij}(0,s) \Veff^{(j)}(t-s) ds
\end{split}
\end{equation}
\normalsize
yields the following expression for $\beta(t,0)$:
\begin{equation}\label{eq:induction_hypo_lemma_tracking_delayed_SDE_beta}
\begin{split}
    \beta^{(i)}(t,x) & = \VSDE^{(i)} \left(t - \frac{1}{\mu_i} \right) \\ 
    \quad & + \int_{t - \frac{1-x}{\mu_i}}^t G_i(0, t-s ) \sigma(s) dW_s
\end{split}
\end{equation}
    where $G_i$ is a deterministic $C^1$ function defined recursively as 
\small
\begin{equation}\label{eq:def_of_G_state_feedback_noise}
\begin{split}
    & G_m(x,u) \triangleq \gamma_\beta^{(m)}( x + \mu_m u )   \\
    & G_i(x,u) \triangleq \gamma_\beta^{(i)}(x + \mu_i u) \\ 
    & + \sum_{j=i+1}^m \int_0^{\overline{s}_{i,j}(x,u)} \omega_{i,j}\bigl (x + \mu_i (u-s) \bigr) G_j \bigl (x + \mu_i (u-s), s \bigr )   ds
\end{split}
\end{equation}
\normalsize
where $\overline{s}_{i,j}(x,u) \triangleq \min \left(  \frac{1-x-\mu_i u}{\mu_j - \mu_i} , u\right)$. 
\end{lemma}

% can we do better with \beta^{(i)}(t,x) = \VSDE \left(t - \frac{1-x}{\mu_i} \right) + \int_{t - \frac{1-x}{\mu_i}}^t G_i(x + \mu_i(t-s)) \sigma(s) dW_s 
\begin{proof}
Inspired by the work of \cite{hu_control_2016}, since $\Omega$ is strictly upper triangular, we operate by induction. We first obtain an explicit expression for $\beta_m(t,x)$, then, for any $i \in [1,m-1]$, we give a formula linking $\beta_i(t,x)$ in terms of other $\beta_j$ for $j \in [i+1,m]$. This allows us to recursively compute $\beta(t,x)$, and then compute a controller $\Veff$ that tracks the desired control $\VSDE$.% The obtained controller $\Veff$ is given by
The details of the proof can be found in the Appendix \ref{APP_LEM_TRACK_NEW}.
\end{proof}
%\modifJA{Je donnerais plutôt le résultat dans l'autre sens. On envoie ce $V_{eff}$ et ça donne ça. En particulier $\beta_i(t,0)=v_i(t,0)$ vérifie... On ne peut pas faire mieux pour des raisons de causalité.}
%In expression \eqref{eq:induction_hypo_lemma_tracking_delayed_SDE_beta}, we do not track the desired controller $\VSDE$ perfectly : it is subject to a delay as well as a noise in the form of a stochastic integral. The delay is due to the finite velocity of propagation of the signal through the transport PDE. If we are to keep an adapted controller (that is one that does not predict future noise), at component $i$ we cannot track at the point $(t,x)$ the signal $\VSDE^{(i)}$ with a delay lower than $\frac{1-x}{\mu_i}$ (as we cannot use future values of $\VSDE^{(i)}$ because then $\Veff$ would not be adapted). We also see in that regard that we cannot compensate the noise any better, as it is given by a stochastic integral between $t - \frac{1-x}{\mu_i}$ and $t$ that is therefore independent of the signal $\VSDE^{(i)}(t - \frac{1-x}{\mu_i})$. 
In expression \eqref{eq:induction_hypo_lemma_tracking_delayed_SDE_beta}, we cannot perfectly track the desired control $\VSDE$; it is affected by both a delay and a stochastic noise term. The delay arises from the finite propagation speed of the signal through the transport PDE. For the component $i$, the control $\VSDE^{(i)}$ cannot be tracked at point $x$ with less delay than $\frac{1-x}{\mu_i}$ without predicting future noise, which would make $\Veff$ non-adapted to the filtration $\mathcal{F}$. Additionally, noise cannot be fully compensated, as it depends on a stochastic integral over  $[t - \frac{1-x}{\mu_i}, t]$, independent from $\VSDE^{(i)}(t - \frac{1-x}{\mu_i})$.


%\commentGV{Write a remark on the fact that the control $\Veff$ cannot better track $\VSDE$ because $\Veff(t-h_i)$ and the stochastic integral $\int_{t-h_i}^t (...) \sigma(s) dW_s $ are independent.}]




\subsection{Well-Posedness and Regularity of the Solution}

%\modifJA{Peut-être donner la tête de celle de $\alpha$?}
Using the explicit expressions for $\alpha$ and $\beta$ given in \eqref{eq:induction_hypo_lemma_tracking_delayed_SDE_beta}, we can now show the well-posedness of the target system directly. 
\begin{lemma}\label{lem:well_posed_SPDE_L2}
    If $\VSDE$ is in $C^2_\mathcal{F}([0,T]; \mathbb{R}^m)$, and $\Veff$ is defined accordingly by \eqref{eq:def_of_Veff_in_terms_of_VSDE}, % \modifJA{dire que $\Veff$ est defini par eq (10)}
    then the closed-loop target system~\eqref{eq:first_target_system_SPDE} is well-posed, that is the processes %\modifJA{Dire ce que ça signifie} 
    $t \mapsto \alpha(t,\cdot)$ and $t \mapsto \beta(t,\cdot)$ are in $C^2_\mathcal{F}([0,T] ; L^2(0,1))$, and the SDE state $X$ is in $C^2_\mathcal{F}([0,T] ; \mathbb{R}^n)$.
\end{lemma}
\begin{proof}
    The proof is identical to the one proposed in~\cite[Lemma 1]{velho_stabilization_2024} for $n=m=1$.
\end{proof}
Since the backstepping transformation is a Volterra transformation, it is boundedly invertible \cite{yoshida_lectures_1960}. This implies the well-posedness of the original system~\eqref{eq:coupled_PDE_SDE}.


\subsection{A delayed SDE}

Lemma \ref{lem:track_VSDE_with_Veff_and_formula_beta} states that for any adapted control $\VSDE$, there exists a controller $\Veff$ such that
$$
\beta(t,0) = \left( \begin{array}{c} \VSDE^{(1)} \left(t - \frac{1}{\mu_1} \right) \\ \vdots \\ \VSDE^{(m)} \left(t - \frac{1}{\mu_m} \right) \end{array} \right) + \int_{t-\frac{1}{\mu_1}}^t G(t-s) \sigma(s) dW_s 
$$
Note that, to streamline notation, we express the noise integral uniformly as $\int_{t-\frac{1}{\mu_1}}^t G(t-s) \sigma(s) dW_s$, where we recall that $\frac{1}{\mu_1}$ represents the largest delay across all components. It is implicitly implied that the components $G_i$ are zero on the intervals  $[\frac{1}{\mu_i}, \frac{1}{\mu_1}]$. This choice avoids detailing each component’s individual delay while capturing the essential structure of the system's noise. 
%Combining these results, we demonstrate that for any desired adapted signal $\VSDE$, we can compute a controller $V(t) = \VPDE + \Veff$, where $\VPDE$ is given by \eqref{eq:expression_backstep_controller} and $\Veff$ is given by \eqref{eq:def_Veff_in_terms_of_VSDE} such that the process 
Consequently, the process $X(t)$ defined in equation~\eqref{eq:coupled_PDE_SDE} is the solution of the following multi-input-delayed stochastic differential equation with random coefficients 
\begin{equation}\label{eq:equivalent_delayed_SDE}
\left\{
\begin{array}{l}
     dX(t) = \left ( A X(t) + \sum_{i=1}^m B_i U_i(t-h_i) + r(t) \right ) dt + \sigma(t) dW_t  \\
     X(0) = X_0, \quad U(s) = \beta(0, 1 + \mu s) \  \forall s \in [-h,0)
\end{array} 
\right.
\end{equation}
where $h_i \triangleq \frac{1}{\mu_{m-i}}$, $U_i \triangleq \VSDE^{(m-i)}$ and %\modifJA{Attention $V_i$ fait trop penser à la $i$ème composante de $V$ peut être l'appeler $\bar V_i$? A moins que ce soit $U$?}
$$
r(t) \triangleq B \int_{t-h_m}^t G(t-s) \sigma(s) dW_s.
$$
Note that we have reversed the components of $\VSDE$ to enhance the clarity of the methods that follow. % \modifJA{Pas très clair}
%\commentGV{Faire un commentaire sur les changements de notations fait ici. Il est important d'inverser les composantes du contrôle pour faciliter la compréhension de la forme de Kalman qui suit.}
%Therefore, we now only focus on controlling the delayed SDE~\eqref{eq:equivalent_delayed_SDE} and minimizing the variance of the state. We follow a methodology similar to the one outlined in \cite{velho_mean-covariance_2023}. However, the inclusion of the extra delays requires to modify our approach to minimize the variance, as the Artstein predictor is more complex.
From now on, we focus on controlling the delayed SDE~\eqref{eq:equivalent_delayed_SDE} and minimizing the state variance. We follow a methodology similar to the one outlined in \cite{velho_mean-covariance_2023}. However, compared to~\cite{velho_mean-covariance_2023}, the additional delays $h_i$ appearing in equation~\eqref{eq:equivalent_multi_delayed_SDE} require extensive non-trivial adjustments in our variance-minimization approach as the computation of Artstein's predictor becomes more complex.










==> 04_5_Stabilization.tex <==


\commentGV{Avant ou après covariance steering? A priori, pas besoin de la forme de Kalmann pour prouver la stabilisation avec "Artstein classique". Mais cela implique introduire un premier prédicteur Arstein ici, pour en donner un autre plus tard. Peut-être que c'est mieux d'inclure cette partie entre la controllabilité et le covariance steering, sinon ça nous pousse à introduire deux types de predicteur d'Artstein, ce qui peut rendre l'article confus.}


















==> 07_Robustness_Comments.tex <==

\


















==> Old_Deprecated_Problem_Formulation.tex <==



\subsection{Notations}

Let us consider $(N,n,m) \in (\mathbb{N} \setminus \{ 0 \})^2$. We assume that state variables take values in $\mathbb{R}^N$, while control variables take values in $\mathbb{R}^m$. 
We assume that we are given a filtered probability space $(\Omega, \mathcal{F} \triangleq (\mathcal{F}_t)_{t \in [0,\infty)}, \mathbb{P})$, %For the sake of clarity in the exposition and without loss of generality, from now on, 
and that stochastic perturbations are due to a one-dimensional Wiener process $W_t$, which is adapted to the filtration $\mathcal{F}$. For clarity, we focus on a one-dimensional Wiener process, noting that all results extend trivially to the multidimensional case but with added notational complexity.
%\textcolor{blue}{Comme dans \cite{yong_stochastic_1999}}. %We denote $\mathcal{F}_t$ the filtration induced by $W_t$.
Let $T > 0$ be some given time horizon. For any $r \in \mathbb{N} \backslash \{0\}$, we denote by $L_\mathcal{F}^2([0,T] , \mathbb{R}^r)$ the set of square-integrable processes $P: [0,T]\times\Omega \to \mathbb{R}^r$ that are $\mathcal{F}$--progressively measurable, whereas the subset $C^2_\mathcal{F}([0,T] , \mathbb{R}^r) \subseteq L_\mathcal{F}^2([0,T] , \mathbb{R}^r)$ contains processes whose sample paths are continuous.
The spaces of semi-definite and definite positive symmetric matrices in $\mathbb{R}^n$ are denoted by $\mathcal{S}^+_n$ and $\mathcal{S}^{++}_n$, respectively. 
If $X \in L_\mathcal{F}^2([0,T] , \mathbb{R}^n)$, we denote by $V_X(\cdot)$ its variance, that is
$
V_X(t) \triangleq \espE[ (X(t) - \espE[X(t)])^T (X(t) - \espE[X(t)]) ] \in \mathbb{R}.
 $ Finally, we recall that if $f_1$ and $f_2$ are two deterministic functions in $L^2([0,T], \mathbb{R})$, It\^o formula yields %then ~\cite{le_gall_brownian_2016} 
 \small
 \begin{align}
     \espE \left[  \left( \int_0^t f_1(s) dW_s  \right) \left( \int_0^t f_2(s) dW_s  \right) \right] = \int_0^t f_1(s) f_2(s) ds. \label{eq:quadratic_variation_of_stochastic_integral}
 \end{align}
\normalsize

Throughout this paper, we consider equalities between stochastic processes up to a modification. This means that the processes are regarded as equal with probability one, even though they may differ on a set of probability zero. This convention is justified by our objective: stabilizing the system in expectation and minimizing variance. As a result, we focus primarily on the expectations of functions of these processes, which are unaffected by modifications. This allows us to simplify expressions without repeatedly noting their equivalence up to modification, thus ensuring clarity and conciseness.

Throughout this paper, we consider equalities between stochastic processes up to a modification. A stochastic process $X$ is a modification of a process $Y$ if $\forall t, \probP(X(t) = Y(t)) = 1$. The expectations are unaffected, as $ \espE[ h(X(t)) ] = \espE[ h(Y(t)) ]$ for any measurable function $h$ such that $\espE[ h(X(t)) ]$ is finite. This convention is justified as we focus primarily on the expectations of functions of the processes (expectation, variance, ... ). This allows us to simplify expressions without repeatedly noting their equivalence up to modification, thus ensuring clarity and conciseness.

%\modifJA{Attention à l'utilisation de Mean/Expectations. Est-ce toujours équivalent?}

\subsection{Equations}

In this paper, we consider interconnected hyperbolic PDE+SDE systems of the form 
%\modifJA{Peut-être redire ici dans quel context ces systèmes peuvent apparaitre?}
\begin{equation}\label{eq:coupled_PDE_SDE}
\left\{
\begin{array}{l}
     dX(t) = ( A X(t) + B v(t,0) ) dt + \sigma(t) dW_t \\
     u_t(t,x) + \Lambda^+ u_x(t,x) = \Sigma^{++}(x) u(t,x) + \Sigma^{+-}(x) v(t,x) \\
     v_t(t,x) - \Lambda^- v_x(t,x) = \Sigma^{-+}(x) u(t,x) + \Sigma^{--}(x) v(t,x) \\
     u(t,0) = Q v(t,0) + M X(t) \\
     v(t,1) = R u(t,1) + \Vin(t) \\
     X(0) = X_0,~ u(0,x) = u_0(x),~ v(0,x) = v_0(x),
\end{array} 
\right.
\end{equation}
in the time-space domain $[0, T] \times [0,1]$, where 
$$
u = (u_1, ... , u_n)^T, \qquad v = (v_1, ... , v_m)^T.
$$
%\modifJA{L'entier $n$ n'a pas été défini jusqu'à présent.} 
The state of the system is $(X(t), u(t,x), v(t,x)) \in \mathbb{R}^N \times L^2([0,1] ; \mathbb{R}^n) \times L^2([0,1] ; \mathbb{R}^m)$. The diagonal matrices $\Lambda^+$ and $\Lambda^-$ are defined as
$$
%\Lambda^+ = \left( \begin{array}{ccc} \lambda_1 & & (0) \\ & \ddots &  \\ (0) & & \lambda_n \end{array} \right), \qquad \Lambda^- = \left( \begin{array}{ccc} \mu_1 & & (0) \\ & \ddots &  \\ (0) & & \mu_m \end{array} \right)
\Lambda^+ = \textrm{diag} \left( \lambda_1, \dots , \lambda_n \right), \quad \Lambda^- = \textrm{diag} \left(   \mu_1, \dots , \mu_m  \right)
$$
%\modifJA{Utilise la convention diag pour les matrices diagonales? Ca permet de gagner un peu de place.}
with 
$$
0 < \lambda_1 < ... < \lambda_n, \qquad 0 < \mu_1 < ... < \mu_m.
$$
These transport velocities are assumed to be constant. However, our results can be extended to space-dependent transport velocities at the cost of technical and lengthy computations. The in-domain coupling terms $\Sigma^{\cdot \cdot}$ are continuous functions. We assume, without loss of generality, that the diagonal entries of $\Sigma^{++}$ and $\Sigma^{--}$ are equal to zero \cite{coron_local_2013}. 
% \modifJA{La ref à mettre est commentée ci-dessous%@article{coron2013local,
%   title={Local exponential H\^{}2 stabilization of a 2$\backslash$times2 quasilinear hyperbolic system using backstepping},
%   author={Coron, Jean-Michel and Vazquez, Rafael and Krstic, Miroslav and Bastin, Georges},
%   journal={SIAM Journal on Control and Optimization},
%   volume={51},
%   number={3},
%   pages={2005--2035},
%   year={2013},
%   publisher={SIAM}
% }
% }
The boundary coupling terms $R$ and $Q$ are such that the open-loop PDE system (i.e. $V_{in}=0$), without the SDE and in the absence of the in-domain coupling terms $\Sigma^{\cdot\cdot}$, is exponentially stable. This condition is required to avoid an infinite number of unstable poles, which is necessary to guarantee the existence of robustness margins for the closed-loop system, see \cite[Theorem 4]{auriol_explicit_2019}.
%The boundary coupling terms $R$ and $Q$ verify $\Vert R Q \Vert < 1$ to avoid an infinite number of unstable poles, which is necessary to guarantee the existence of robustness margins for the closed-loop system \cite{auriol_delay-robust_2018} 
%\modifJA{Pas tout à fait la bonne condition en vectoriel. Il faudrait plutôt dire: "The boundary coupling terms $R$ and $Q$ are such that the open-loop PDE system (i.e. $V_{in}=0$) without the SDE and in the absence of the in-domain coupling terms $\Sigma^{\cdot\cdot}$ is exponentially stable. This condition is required to avoid an infinite number of unstable poles, which is necessary to guarantee the existence of robustness margins for the closed-loop system" et citer le Théorème 4 de mon papier 2019 avec Florent (explicit mapping)}
%\commentGV{Attention est ce que c'est la bonne condition pour les dimensions $> 1$?}.
%We also assume $Q \neq 0$ \commentGV{Idem, a changer, check transformations}. 
The matrices $A \in \mathbb{R}^{N\times N}, B \in \mathbb{R}^{N\times m}, M \in \mathbb{R}^{n\times N}$ are constant, and~$\sigma$ is a deterministic diffusion in $L^\infty([0,T], \mathbb{R}^N)$. Finally, $(X_0, u_0, v_0) \in \chi$ with $\chi \triangleq \mathbb{R}^N \times L^2([0,1] ; \mathbb{R}^n) \times L^2([0,1] ; \mathbb{R}^m)$ the space our state evolves in. The control input $V$ is in the space $L_{\mathcal{F}}^2([0,T] ; \mathbb{R}^m)$.
%\modifJA{Attention est-ce $V$ on $V_{in}$. Il faut être cohérent dans les notations.}
The class of system~\eqref{eq:coupled_PDE_SDE} naturally appear, for example, when modeling a heat-exchanger connected to a temperature system subject to random perturbations (e.g., the temperature of a building disrupted by a random outside temperature or sunlight).
We make the following classic controllability assumption on the dynamic in order to effectively control the system.
\begin{assumption}\label{ass:controlability_of_the_SDE}
The pair of matrices $(A, (B_1, \dots , B_m) )$ is controllable.    
\end{assumption}
The well-posedness of the system is proved in section \ref{TRA} after the backstepping change of variable, where we show that the state $(X(\cdot), u(\cdot , \cdot), v(\scot, \cdot))$ is in $L^2_\mathcal{F}(\chi)$
%\modifJA{Préciser qu'on montrera que l'état restera dans $\mathbb{R}^N \times L^2([0,1] ; \mathbb{R}^n) \times L^2([0,1] ; \mathbb{R}^m)$. Peut-être donner un nom du genre $\chi=\mathbb{R}^N \times L^2([0,1] ; \mathbb{R}^n) \times L^2([0,1] ; \mathbb{R}^m)$ pour éviter de réécrire ce domain 36 fois.}




%\subsection{Assumptions}

%\begin{assumption}
%    We assume the pair of matrices $(A,B)$ to be controllable.
%\end{assumption}

%\begin{assumption}
%    We assume the pair of matrices $(A,(B_1, ... , B_m))$ to be controllable but not $(A,(B_1, ... , B_{m-1}))$.
%\end{assumption}


%\subsection{Well-Posedness}

%The well-posedness is studied after the backstepping feedback loop is presented. Indeed, the study of the target equation is easier than the original system.



\subsection{Objective}
The system \eqref{eq:coupled_PDE_SDE} naturally contains multiple feedback loops or couplings that can potentially introduce instabilities. Therefore our objective is three-fold:
%\modifJA{Avant de décrire l'objectif, peut-être souligner les prbolèmes qui apparaissent en Open-loop? "The system naturally contains multiple feedback loops or couplings that can potentially introduce instabilities. Therefore our objective is three-fold"}
%Our objective is three-fold :
%\modifJA{Que veut dire straightforward? Mot un peu vide de sens. Veux-tu dire explicit?} 
\begin{enumerate}
    \item Analyze controllability and variance steering: We establish a structural lower bound on the achievable variance of the SDE state for any control strategy. Additionally, we show that open-loop controls can steer the variance arbitrarily close to this minimal bound.
    \item Stabilize the PDE+SDE system with feedback control: Since open-loop controls are generally impractical due to the unobservable noise realizations $ dW_t $ \cite{touzi_introduction_2013}, we give a stabilizing feedback law. This stabilizes the coupled PDE+SDE system by driving the expectation of the state to zero with exponential convergence while keeping the variance bounded. Specifically, for  $x \in [0,1]$ and $t>\frac{1}{h_m}$, the state $(X,u,v)$ satisfies:
    \begin{equation}\label{eq:stabilization_mean_expectation}
    \begin{split}
    &  \Vert \espE[X(t)] \Vert + \Vert \espE[u(x,t)] \Vert + \Vert \espE[v(x,t)] \Vert \leq C e^{- \nu t} \times\\
   & \quad \times \bigl (\Vert \espE[X_0] \Vert + \Vert  \espE [u_0] \Vert + \Vert  \espE [v_0] \Vert \bigr ), \\
   &  \espE \left[ \Vert X(t)\Vert^2 \right]  + \espE \left[ \Vert u(x,t) \Vert^2 \right] + \espE \left[ \Vert v(x,t) \Vert^2 \right] \leq C
    \end{split}
    \end{equation}
    with $C>0$ depends on the system parameters, and $\nu$ is determined by the feedback gain.
    
    \item We design a control that minimizes the quadratic cost of the SDE state while penalizing control input at the boundary
    \begin{align*}
    J(X, v(t,0) ) \triangleq & \ \espE \left[  \int_0^T X(t)^T Q(t) X(t)  \right. \\
    & \hspace{3em} + \left. \int_0^T v(t,0)^T R(t) v(t,0) \right]. 
    \end{align*}
    This approach minimizes the variance, enhancing robustness to perturbations and remaining computationally feasible. Under standard controllability assumptions, this strategy achieves variance arbitrarily close to the theoretical minimum by reducing the penalty parameter $R$ toward zero.
\end{enumerate}

%\modifJA{Je pense qu'on peut mieux exprimer ces objectifs. On en discute ensemble.}




































==> copy_old_track_problem.tex <==





In system \eqref{eq:coupled_PDE_SDE}, the in-domain coupling terms $\Sigma^{\cdot\cdot}$ in the PDE can cause instabilities and disrupt the control of the SDE \cite{auriol_delay-robust_2018}. %\modifJA{Mettre une citation?}. 
Therefore, we will first apply a backstepping transformation to move these coupling terms to the boundary at $x=1$, where the control input is applied. Then, we will design the input $V(t)$ as a sum of two control components: $V(t)=\VPDE(t)+\Veff(t)$. The term $\VPDE(t)$ will correspond to a classical backstepping control input,  used to cancel the (potentially) unstable coupling terms appearing at the controlled boundary. It would stabilize the PDE in the absence of the SDE. On the other hand, $\Veff(t)$ is the effective control that propagates through the PDE, allowing us to track a desired signal entering the SDE.

%\modifJA{J'ai bougé la fin ailleurs car ça faisait trop de choses à assimiler.}



%\subsection{Transformation into a Target System}
%\subsubsection{The Backstepping Transformation}
%\subsubsection{Existence of a Solution of the Kernel Equations}

\subsection{The Backstepping Transformation}

Taking inspiration from \cite{auriol_delay-robust_2018}, we consider the following backstepping change of variables:

\begin{equation}\label{eq:backstepping_transform_alpha_beta_definition}
 \begin{split}
 \alpha(t,x) \triangleq u(t,x) & + \int_0^x K_{uu}(x,y) u(t,y) dy \\ 
 & + \int_0^x K_{uv}(x,y) v(t,y) dy + \gamma_\alpha(x) X(t) \\
 \beta(t,x) \triangleq v(t,x) & + \int_0^x K_{vu}(x,y) u(t,y) dy \\ 
 & + \int_0^x K_{vv}(x,y) v(t,y) dy + \gamma_\beta(x) X(t).
 \end{split}
\end{equation}
The kernels  $K_{uu}, K_{uv}, K_{vu}$, and $K_{vv}$ are piecewise continuous functions defined on the triangular domain $\mathcal{T} \triangleq \left\{ (x,y), x \in [0,1], y \in [0,x]  \right\}$, whereas $\gamma_\alpha, \gamma_\beta$ are in $C^1([0,1] ; \mathbb{R}^{n \times N}) \times C^1([0,1] ; \mathbb{R}^{m \times N})$. On their respective domains of definition, $K$ and $\gamma$ verify the following set of \textit{kernel equations}: 

%\commentGV{Changement d'ordre par rapport à CDC, on introduit d'abord le target système pour introduire les fonctions $\Psi$ et $\Omega$.}





 \begin{equation}\label{eq:kernel_equations_alpha}
 \left\{
 \begin{array}{l}
      \Lambda^+ (K_{uu})_x(x,y) + (K_{uu})_y(x,y) \Lambda^+ \\ 
      \quad + K_{uu}(x,y) \Sigma^{++}(y) + K_{uv}(x,y) \Sigma^{-+}(y) = \Psi(x) K_{uu}(x,y) \\
      \Lambda^+ (K_{uv})_x(x,y) - (K_{uv})_y(x,y) \Lambda^- \\
      \quad + K_{uu}(x,y) \Sigma^{+-}(y) + K_{uv}(x,y) \Sigma^{--}(y) =  \Psi(x) K_{uv}(x,y) \\
      \Lambda^+  K_{uu}(x,x) - K_{uu}(x,x) \Lambda^+ + \Sigma^{++}(x) = 0 \\
      \Lambda^+  K_{uv}(x,x) + K_{uv}(x,x) \Lambda^- + \Sigma^{+-}(x) = 0 \\
      K_{uu}(x,0) \Lambda^+ Q - K_{uv}(x,0) \Lambda^- + \gamma_\alpha(x) B = \Psi(x)  \\
      \Lambda^+ \gamma_\alpha'(x) + \gamma_\alpha(x) A + K_{uu}(x,0) \Lambda^+ M  = 0 \\
      \gamma_\alpha(0) = -M,
 \end{array} 
 \right.
 \end{equation}
 as well as
\modifJA{S'il faut gagner de la place, on pourra utiliser la forme condensée proposée dans LCSS ou mon papier Automatica de 2023 (robustification of ...)} \begin{equation}\label{eq:kernel_equations_beta}
 \left\{
 \begin{array}{l}
      - \Lambda^- (K_{vu})_x(x,y) + (K_{vu})_y(x,y) \Lambda^+ \\
      \quad + K_{vu}(x,y) \Sigma^{++}(y) + K_{vv}(x,y) \Sigma^{-+}(y) = \Omega(x) K_{vu}(x,y) \\
      - \Lambda^- (K_{vv})_x(x,y) - (K_{vv})_y(x,y) \Lambda^- \\
      \quad + K_{vu}(x,y) \Sigma^{+-}(y) + K_{vv}(x,y) \Sigma^{++}(y) = \Omega(x) K_{vv}(x,y) \\
      - \Lambda^-  K_{vu}(x,x) - K_{vu}(x,x) \Lambda^+ + \Sigma^{-+}(x) = 0 \\
      - \Lambda^-  K_{vv}(x,x) + K_{vv}(x,x) \Lambda^- + \Sigma^{--}(x) = \Omega(x) \\
      K_{vu}(x,0) \Lambda^+ Q - K_{vv}(x,0) \Lambda^- + \gamma_\beta(x) B = 0 \\
      - \Lambda^- \gamma_\beta'(x) + \gamma_\beta(x) A  + K_{vu}(x,0) \Lambda^+ M = 0 \\
      \gamma_\beta(0) = 0.
 \end{array} 
 \right.
 \end{equation}
%\commentGV{retrouver ou interviennent $\Psi$ et $\Omega$, les équations ne sont pas bien posées telles qu'elles sont.}
where $\Psi$ and $\Omega$ are two strict upper triangular matrices. %of the form \modifJA{Pas nécessaire de metttre explicitement les matrices. Tu dis déjà qu'elles sont trig. sup.}
% \small
% $$
% \Psi(x) = \left( \begin{array}{ccc} 0 & & (\psi(x))_{i,j} \\ & \ddots &  \\ (0) & & 0 \end{array} \right),  \Omega(x) = \left( \begin{array}{ccc} 0 & & (\omega(x)))_{i,j} \\ & \ddots &  \\ (0) & & 0 \end{array} \right).
% $$
% \normalsize
Their coefficients verify
\begin{align*}
\psi_{i,j}(x) & =  ( \lambda_i - \lambda_j) K_{uu}(x,x)_{i,j} + \Sigma^{++}_{i,j} \\
\omega_{i,j}(x) & = ( \mu_j - \mu_i) K_{vv}(x,x)_{i,j} + \Sigma^{--}_{i,j}.
\end{align*}
The set of equations \eqref{eq:kernel_equations_alpha}-\eqref{eq:kernel_equations_beta}is well posed and admits a unique solution \cite{auriol_minimum_2016, di_meglio_stabilization_2018}. % \modifJA{Il faudrait faire référence au numéro d'équations. Par ailleurs in me semble qu'il y a un problème de conditions de bords pour $K_{uu}(x,0)$. Ca pourrait avoir des conséquence importantes sur le système cible (mais mineures sur le reste du papier). Il faudrait je pense remplacer $\Psi(x)\alpha(t,x)$ par $\Psi(x)\beta(t,0)$ En ref, il faut aussi citer le papier de Di Meglio/Hu/Bribiesca-Argomedo/Krstic (gestion du term ODE).}
By setting our stabilizing backstepping controller as 
\begin{equation}\label{eq:definition_expression_backstep_controller}
\begin{split}
& \VPDE(t) = - R u(t,1) - \gamma_\beta(1) X(t) \\
    & \ - \int_0^1 K_{vu}(1,y) u(t,y) dy - \int_0^1 K_{vv}(1,y) v(t,y) dy.
\end{split}
\end{equation}
and by differentiating with respect to time and space (in the sense of distributions), and integrating by parts, we can show that the states $(\alpha,\beta,X)$ are solutions to the following \textit{target system}:
\begin{equation}\label{eq:first_target_system_SPDE}
\left\{
\begin{array}{l}
     dX(t) = ( A X(t) + B \beta(t,0) ) dt + \sigma(t) dW_t \\
     d \alpha(t,x) + \Lambda^+ \alpha_x(t,x) = \Psi(x)\beta(t,0) + \gamma_\alpha(x) \sigma(t) dW_t \\
     d \beta(t,x) - \Lambda^- \beta_x(t,x) = \Omega(x) \beta(t,x) + \gamma_\beta(x) \sigma(t) dW_t \\
     \alpha(t,0) = Q \beta(t,0), \ \beta(t,1) = \Veff(t) 
\end{array} 
\right.
\end{equation}

%\modifJA{Mettre ce qui suit en remarque:
In the absence of the SDE, this target system would be exponentially stable. However, due to the cancellation of the term $Ru(t,1)$, the feedback operator induced by $\VPDE$ is not strictly proper. This could lead to (delay)-robustness issues, as highlighted in~\cite{auriol_delay-robust_2018}. To address these concerns, different approaches have been proposed as partial cancellation of the reflection~\cite{auriol_delay-robust_2018} or filtering methods~\cite{auriol_robustification_2023}. However, these methods do not directly adapt to the current stochastic configuration. Specifically, we should be able to show robust mean square stability, but quantifying the impact of these techniques on variance proves to be challenging. This robustness analysis is beyond the scope of this paper and is left for future research.
%}

%\revAns{Attention à introduire Vin, Veff et VBS comme dans CDC dans le problem formulation.}

%\subsection{Signal Tracking}

%Although the coupling between $u$ and $v$ is handled, there remain cascading interactions between the states $v^{(i)}(t,x)$ and $v^{(j)}(t,x)$ for $i>j$. 
%Additionally, we need to account for the interaction from the SDE back into the PDE. 
While system \eqref{eq:first_target_system_SPDE} is simpler to handle, expressing $\beta(t,0)$ in terms of $\Veff$ remains complex, complicating the task of tracking a desired control through the PDE into the SDE. In what follows, we show how we can further simplify system   \eqref{eq:first_target_system_SPDE} into a input-delayed SDE, with an arbitrary input $\VSDE \in L^2_\mathcal{F}([0,T] ; \mathbb{R}^m)$ by choosing an appropriate controller $\Veff$.
%We therefore show that, for any desired signal $V_{SDE}(t)$ in $L^2_\mathcal{F}([0,T] ; \mathbb{R}^m)$ that we want to track into the SDE,  $\Veff(t)$ can be chosen to ensure the boundary condition $v^{(i)}(t,0) = V_{SDE}^{(i)}(t-\frac{1}{\mu_i}) + \int_{t - \frac{1}{\mu_i}}^t G_i(t-s ) \sigma(s) dW_s $ is met. The delay reflects the finite control velocity, and the stochastic integral arises from the noise that cannot be canceled.
%\modifJA{$\VSDE$ n'est pas proprement défini. On ne comprend pas à quoi ça correspond.}


\subsection{Solving the SPDE Through the Characteristic Method}
\modifJA{Balise à garder pour me rappeler de relire cette section une fois modifiée.}


To achieve our desired control behavior at the boundary of the SDE, we start by considering an input $\Veff$ applied to the PDE. Due to the coupling terms within the PDE in system \eqref{eq:first_target_system_SPDE}, this input does not directly translate to a simple expression for $\beta(t,0)$. However, we find that by choosing $\Veff$ in a specific form relative to an arbitrary process $S(t) \in L^2_\mathcal{F}([0,T] ; \mathbb{R}^m)$, we obtain a clean boundary condition at the other end of the PDE $\beta^{(i)}(t,0) = S^{(i)}(t-\frac{1}{\mu_i}) + \int_{t - \frac{1}{\mu_i}}^t G_i(t-s ) \sigma(s) dW_s $.
This result implies that any desired control $\VSDE$ can be approximately tracked at $\beta(t,0)$ when choosing $S(t) = \VSDE(t)$. 
%We cannot track the process any better, as the delay reflects the finite control velocity, and the stochastic integral arises from the noise that cannot be canceled.
%We can now solve through the characteristic method and the Ito formula the SPDE \eqref{eq:first_target_system_SPDE}. As mentioned previously, this allows us to compute an effective control $\Veff$ that tracks a desired control $\VSDE$ into the SDE.
%For clarity and conciseness, we only do this for $\beta$. %, although a very similar formula can be obtained for $\alpha$.
%\modifJA{Paragraphe peu clair. A reformuler. Pourquoi on a besoin de celle de $\alpha$?}
%\commentGV{A REVOIR: l'expression du contrôle $\Veff$ ne peut pas dépendre de $x$! Il faut en fait prendre l'expression en $x=0$. Le problème c'est que l'expression de $\beta(t,x)$ va changer sur le reste du domaine et on aura une induction qui sera plus complexe que ça. La méthode reste correcte, mais l'expression de $\Veff$ est beaucoup plus compliqué.}
\commentGV{A REVOIR: Le contrôleur proposé n'est pas causal, il faut revoir la preuve et affiner l'expression de $\beta$.      }
\begin{lemma}\label{lem:track_VSDE_with_Veff_and_formula_beta}
    Let $\VSDE$ be a $ L^2_\mathcal{F}([0,T] ; \mathbb{R}^m)$ controller we want to track into the SDE. %\modifJA{Qu'est-ce que ça veut dire ? Il faut introduire $\VSDE$ plus clairement et proprement.} 
    The input $\Veff \in  L^2_\mathcal{F}([0,T] ; \mathbb{R}^m)$ recursively defined as 
    %such that \modifJA{Domaine de $t$ et $x$?}
    \small
\begin{equation}\label{eq:def_of_Veff_in_terms_of_VSDE}
\begin{split}
% &  \Veff^{(m)}(t)  = \VSDE^{(m)}(t)   \\
% & \Veff^{(i)}(t)  = \VSDE^{(i)} \left(t \right) \\
% & - \sum_{j=i+1}^m  \int_{0}^{\frac{1-x}{\mu_i}} \omega_{i,j}(x + \mu_i s ) \times \\
% & \hspace{6em} \VSDE^{(j)} \left(t + \frac{1-x}{\mu_i} + s - \frac{1 - x - \mu_i s}{\mu_j} \right)  ds 
\Veff^{(i)}(t- \frac{1}{\mu_i} ) & = \VSDE^{(i)}(t- \frac{1}{\mu_i} ) \\
& -  \sum_{j=i+1}^m \int_0^{\frac{1}{\mu_i}} F_{ij}(0,s) \Veff^{(j)}(t-s) ds
\end{split}
\end{equation}
\normalsize
yields the following expression for $\beta(t,0)$:
\begin{equation}\label{eq:induction_hypo_lemma_tracking_delayed_SDE_beta}
\begin{split}
    \beta^{(i)}(t,x) & = \VSDE^{(i)} \left(t - \frac{1}{\mu_i} \right) \\ 
    \quad & + \int_{t - \frac{1-x}{\mu_i}}^t G_i(0, t-s ) \sigma(s) dW_s
\end{split}
\end{equation}
    where $G_i$ is a deterministic $C^1$ function defined recursively as 
\small
\begin{equation}\label{eq:def_of_G_state_feedback_noise}
\begin{split}
    & G_m(x,u) \triangleq \gamma_\beta^{(m)}( x + \mu_m u )   \\
    & G_i(x,u) \triangleq \gamma_\beta^{(i)}(x + \mu_i u) \\ 
    & + \sum_{j=i+1}^m \int_0^{\overline{s}_{i,j}(x,u)} \omega_{i,j}\bigl (x + \mu_i (u-s) \bigr) G_j \bigl (x + \mu_i (u-s), s \bigr )   ds
\end{split}
\end{equation}
\normalsize
where $\overline{s}_{i,j}(x,u) \triangleq \min \left(  \frac{1-x-\mu_i u}{\mu_j - \mu_i} , u\right)$. 
\end{lemma}

% can we do better with \beta^{(i)}(t,x) = \VSDE \left(t - \frac{1-x}{\mu_i} \right) + \int_{t - \frac{1-x}{\mu_i}}^t G_i(x + \mu_i(t-s)) \sigma(s) dW_s 
\begin{proof}
Inspired by the work of \cite{hu_control_2016}, since $\Omega$ is strictly upper triangular, we operate by induction. We first obtain an explicit expression for $\beta_m(t,x)$, then, for any $i \in [1,m-1]$, we give a formula linking $\beta_i(t,x)$ in terms of other $\beta_j$ for $j \in [i+1,m]$. This allows us to recursively compute $\beta(t,x)$, and then compute a controller $\Veff$ that tracks the desired control $\VSDE$.% The obtained controller $\Veff$ is given by
The details of the proof can be found in the Appendix \ref{APP_LEM_TRACK_NEW}.
\end{proof}
%\modifJA{Je donnerais plutôt le résultat dans l'autre sens. On envoie ce $V_{eff}$ et ça donne ça. En particulier $\beta_i(t,0)=v_i(t,0)$ vérifie... On ne peut pas faire mieux pour des raisons de causalité.}
%In expression \eqref{eq:induction_hypo_lemma_tracking_delayed_SDE_beta}, we do not track the desired controller $\VSDE$ perfectly : it is subject to a delay as well as a noise in the form of a stochastic integral. The delay is due to the finite velocity of propagation of the signal through the transport PDE. If we are to keep an adapted controller (that is one that does not predict future noise), at component $i$ we cannot track at the point $(t,x)$ the signal $\VSDE^{(i)}$ with a delay lower than $\frac{1-x}{\mu_i}$ (as we cannot use future values of $\VSDE^{(i)}$ because then $\Veff$ would not be adapted). We also see in that regard that we cannot compensate the noise any better, as it is given by a stochastic integral between $t - \frac{1-x}{\mu_i}$ and $t$ that is therefore independent of the signal $\VSDE^{(i)}(t - \frac{1-x}{\mu_i})$. 
In expression \eqref{eq:induction_hypo_lemma_tracking_delayed_SDE_beta}, we cannot perfectly track the desired control $\VSDE$; it is affected by both a delay and a stochastic noise term. The delay arises from the finite propagation speed of the signal through the transport PDE. For the component $i$, the control $\VSDE^{(i)}$ cannot be tracked at point $x$ with less delay than $\frac{1-x}{\mu_i}$ without predicting future noise, which would make $\Veff$ non-adapted to the filtration $\mathcal{F}$. Additionally, noise cannot be fully compensated, as it depends on a stochastic integral over  $[t - \frac{1-x}{\mu_i}, t]$, independent of $\VSDE^{(i)}(t - \frac{1-x}{\mu_i})$.


%\commentGV{Write a remark on the fact that the control $\Veff$ cannot better track $\VSDE$ because $\Veff(t-h_i)$ and the stochastic integral $\int_{t-h_i}^t (...) \sigma(s) dW_s $ are independent.}]




\subsection{Well-Posedness and Regularity of the Solution}

%\modifJA{Peut-être donner la tête de celle de $\alpha$?}
Using the explicit expressions for $\alpha$ and $\beta$ given in \eqref{eq:induction_hypo_lemma_tracking_delayed_SDE_beta}, we can now demonstrate the well-posedness of the target system directly. 
\begin{lemma}\label{lem:well_posed_SPDE_L2}
    If $\VSDE$ is in $C^2_\mathcal{F}([0,T]; \mathbb{R}^m)$, and $\Veff$ is defined accordingly by \eqref{eq:def_of_Veff_in_terms_of_VSDE}, % \modifJA{dire que $\Veff$ est defini par eq (10)}
    then the closed-loop target system~\eqref{eq:first_target_system_SPDE} is well-posed, that is the processes %\modifJA{Dire ce que ça signifie} 
    $t \mapsto \alpha(t,\cdot)$ and $t \mapsto \beta(t,\cdot)$ are in $C^2_\mathcal{F}([0,T] ; L^2(0,1))$, and the SDE state $X$ is in $C^2_\mathcal{F}([0,T] ; \mathbb{R}^n)$.
\end{lemma}
\begin{proof}
    The proof is identical to the one proposed in~\cite[Lemma 1]{velho_stabilization_2024} for $n=m=1$.
\end{proof}
Since the backstepping transformation is a Volterra transformation, it is boundedly invertible \cite{yoshida_lectures_1960}. This implies the well-posedness of the original system~\eqref{eq:coupled_PDE_SDE}.


\subsection{A delayed SDE}

Lemma \ref{lem:track_VSDE_with_Veff_and_formula_beta} states that for any adapted control $\VSDE$, there exists a controller $\Veff$ such that
$$
\beta(t,0) = \left( \begin{array}{c} \VSDE^{(1)} \left(t - \frac{1}{\mu_1} \right) \\ \vdots \\ \VSDE^{(m)} \left(t - \frac{1}{\mu_m} \right) \end{array} \right) + \int_{t-\frac{1}{\mu_1}}^t G(t-s) \sigma(s) dW_s 
$$
Note that, to streamline notation, we express the noise integral uniformly as $\int_{t-\frac{1}{\mu_1}}^t G(t-s) \sigma(s) dW_s$, where we recall that $\frac{1}{\mu_1}$ represents the largest delay across all components. It is implicitly implied that the components $G_i$ are zero on the intervals  $[\frac{1}{\mu_i}, \frac{1}{\mu_1}]$. This choice avoids detailing each component’s individual delay while capturing the essential structure of the system's noise. 
%Combining these results, we demonstrate that for any desired adapted signal $\VSDE$, we can compute a controller $V(t) = \VPDE + \Veff$, where $\VPDE$ is given by \eqref{eq:expression_backstep_controller} and $\Veff$ is given by \eqref{eq:def_Veff_in_terms_of_VSDE} such that the process 
Consequently, the process $X(t)$ defined in equation~\eqref{eq:coupled_PDE_SDE} is the solution of the following multi-input-delayed stochastic differential equation with random coefficients 
\begin{equation}\label{eq:equivalent_delayed_SDE}
\left\{
\begin{array}{l}
     dX(t) = \left ( A X(t) + \sum_{i=1}^m B_i U_i(t-h_i) + r(t) \right ) dt + \sigma(t) dW_t  \\
     X(0) = X_0, \quad U(s) = \beta(0, 1 + \mu s) \  \forall s \in [-h,0)
\end{array} 
\right.
\end{equation}
where $h_i \triangleq \frac{1}{\mu_{m-i}}$, $U_i \triangleq \VSDE^{(m-i)}$ and %\modifJA{Attention $V_i$ fait trop penser à la $i$ème composante de $V$ peut être l'appeler $\bar V_i$? A moins que ce soit $U$?}
$$
r(t) \triangleq B \int_{t-h_m}^t G(t-s) \sigma(s) dW_s.
$$
Note that we have reversed the components of $\VSDE$ to enhance the clarity of the methods that follow. % \modifJA{Pas très clair}
%\commentGV{Faire un commentaire sur les changements de notations fait ici. Il est important d'inverser les composantes du contrôle pour faciliter la compréhension de la forme de Kalman qui suit.}
%Therefore, we now only focus on controlling the delayed SDE~\eqref{eq:equivalent_delayed_SDE} and minimizing the variance of the state. We follow a methodology similar to the one outlined in \cite{velho_mean-covariance_2023}. However, the inclusion of the extra delays requires to modify our approach to minimize the variance, as the Artstein predictor is more complex.
From now on, we focus on controlling the delayed SDE~\eqref{eq:equivalent_delayed_SDE} and minimizing the state variance. We follow a methodology similar to the one outlined in \cite{velho_mean-covariance_2023}. However, compared to~\cite{velho_mean-covariance_2023}, the additional delays $h_i$ appearing in equation~\eqref{eq:equivalent_delayed_SDE} induce adjustments in our variance-minimization approach as the computation of Artstein's predictor becomes more complex.



















==> unused_latex_code.tex <==



%%% Proof with delays, maybe not the best approach
\subsection{Proof of theorem \ref{thm:Kalman_canonical_extended}}
This theorem is an extension of the Kalmann canonical form theorem that states
\begin{theorem}\label{thm:Kalmann_canonical_base}
    Let $A \in \mathbb{R}^{n \times n} $ and $B \in \mathbb{R}^{n \times m} $ be two matrices, and let $X$ be the process defined by
    $$
    \dot{X} = AX + BU
    $$
    then there exists a reversible matrix $M$ such that $Z \triangleq M X$ verifies
$$
\dot{Z} = \left( \begin{array}{cc} \overline{A}_{11} & \overline{A}_{12} \\ 0 & \overline{A}_{22} \end{array} \right) Z + \left( \begin{array}{c} \overline{B}_{11} \\ 0 \end{array} \right) U
$$
with $\overline{A} = M A M^{-1}$, $\left( \begin{array}{c} \overline{B}_{11} \\ 0 \end{array} \right) = M B$, and $(\overline{A}_{11} , \overline{B}) $ controllable.
\end{theorem}
We now prove the extension presented in theorem \ref{thm:Kalman_canonical_extended}.

\begin{proof}
We proceed by induction on $m$. For $m=1$, the theorem \ref{thm:Kalman_canonical_extended} is true without any change of variable. Suppose now that the property is true for any $m' < m$. Suppose that $X$ follows the dynamic
$$
\dot{X}(t) = A X(t) + \sum_{i=1}^m B_i U_i(t-h_i),
$$
with $(A, (B_1, ... , B_m) )$ controllable. Kalmann canonical form theorem \ref{thm:Kalmann_canonical_base} applied to matrices $A$ and $B_1$ states that there exists a matrix $M_1$ such that $Z^{(1)} \triangleq M_1 X$ verifies
\small
\begin{align*}
& \dot{Z}^{(1)}(t)  = \left( \begin{array}{c | c} \overline{A}^{(1)}_{11} & \left( \overline{A}^{(1)}_{12}, ..., \overline{A}^{(1)}_{1m}  \right) \\ \hline \left( \begin{array}{c} 0 \\ \vdots \\ 0 \end{array} \right) & \overline{A}^{(1)}_2 \end{array} \right) \left( \begin{array}{c} Z^{(1)}_1(t) \\ \left( \begin{array}{c} Z^{(1)}_2(t) \\ \vdots \\ Z^{(1)}_m(t) \end{array} \right) \end{array} \right) \\
& \ +  \left( \begin{array}{c | c} \overline{B}^{(1)}_{11} & \left( \overline{B}^{(1)}_{12}, ..., \overline{B}^{(1)}_{1m}  \right) \\ \hline \left( \begin{array}{c} 0 \\ \vdots \\ 0 \end{array} \right) & \overline{B}^{(1)}_2 \end{array} \right) \left( \begin{array}{c} U_1(t-h_1) \\ \left( \begin{array}{c} U_2(t-h_2) \\ \vdots \\ U_m(t-h_m) \end{array} \right) \end{array} \right),
\end{align*}
\normalsize
with $(\overline{A}^{(1)}_{11}, \overline{B}^{(1)}_{11}) $ controllable. Since the change of variable is reversible, 




\end{proof}
